Spectral Experts for Estimating Mixtures of Linear Regressions

Discriminative latent-variable models are typically learned using EM or gradient-based optimization, which suffer from local optima. In this paper, we develop a new computationally efficient and provably consistent estimator for a mixture of linear regressions, a simple instance of a discriminative latent-variable model. Our approach relies on a low-rank linear regression to recover a symmetric tensor, which can be factorized into the parameters using a tensor power method. We prove rates of convergence for our estimator and provide an empirical evaluation illustrating its strengths relative to local optimization (EM).

==> pdiag-macros.tex <==
% Perturbation Diagram TikZ Macros

% Some style definitions
\tikzstyle{block} = [rectangle, draw, text centered]
\tikzstyle{line} = [draw, -latex]
\tikzstyle{vec} = [draw, -latex, dashed]
\tikzstyle{mmat} = [draw, -latex, double]
\tikzstyle{mvec} = [draw, -latex, double, dashed]
\tikzstyle{tensor} = [draw, -latex, dashdotted]

% First argument is name, second is location specifier
\newcommand{\addb}[2] { \node[block, #2] (#1) {$+$}; }
\newcommand{\mulb}[2] { \node[block, #2] (#1) {$*$}; }
\newcommand{\invb}[2] { \node[block, #2] (#1) {$-1$}; }
\newcommand{\eigb}[2] { \node[block, #2] (#1) {$\lambda$}; }
\newcommand{\evecb}[2] { \node[block, #2] (#1) {$\xi$}; }
\newcommand{\svecb}[2] { \node[block, #2] (#1) {$\nu$}; }
\newcommand{\rotb}[2] { \node[block, #2] (#1) {$\circlearrowright$}; }
\newcommand{\whiteb}[2] { \node[block, #2] (#1) {$W$}; }
\newcommand{\innerb}[2] { \node[block, #2] (#1) {$\triangleleft$}; }

\newcommand{\pdiagadd}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A$};
  \node[right of=a] (ab) {};
  \node[right of=ab] (b) {$B$};
  \addb{a+b}{below of=ab};

  \path[line] (a) -| (a+b);
  \path[line] (b) -| (a+b);
\end{tikzpicture}
}

\newcommand{\pdiagmul}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A$};
  \node[right of=a] (ab) {};
  \node[right of=ab] (b) {$B$};
  \mulb{c}{below of=ab};

  \path[line] (a) -| (c);
  \path[line] (b) -| (c);
\end{tikzpicture}
}

\newcommand{\pdiaginv}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A$};
  \invb{b}{below of=a};

  \path[line] (a) -- (b);
\end{tikzpicture}
}

\newcommand{\pdiageig}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A$};
  \eigb{b}{below of=a};

  \path[line] (a) -- (b);
\end{tikzpicture}
}

\newcommand{\pdiageign}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A_1 \ldots A_n$};
  \eigb{b}{below of=a};

  \path[line] (a) -- (b);
\end{tikzpicture}
}

\newcommand{\pdiagevec}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A$};
  \evecb{b}{below of=a};

  \path[line] (a) -- (b);
\end{tikzpicture}
}

\newcommand{\pdiagsvec}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A$};
  \svecb{b}{below of=a};

  \path[line] (a) -- (b);
\end{tikzpicture}
}

\newcommand{\pdiagrot}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A$};
  \node[right of=a] (b) {$B$};
  \rotb{c}{below of=a};

  \path[line] (a) -- (c);
  \path[line] (b) |- (c);
\end{tikzpicture}
}

\newcommand{\pdiagwhite}{
\begin{tikzpicture}[node distance=1cm,auto]
  \node (a) {$A$};
  \node[right of=a] (b) {$B$};
  \whiteb{c}{below of=a};

  \path[line] (a) -- (c);
  \path[line] (b) |- (c);
\end{tikzpicture}
}



==> tensor-power.tex <==
%\subsection{Tensor Factorization}
%\label{sec:tensor-power}
%
%%Write out the form of $B$ and $\mathcal{B}$ in symmetric tensor form.
%
%%Use Tensor Power Method to recovery $\beta_k$.
%
%By 
%
%\begin{lemma}
%  Let $\hat T = T + E$, where $T$ is a symmetric tensor with orthogonal decomposition $T = \sum_{i=1}^k \lambda_i v_i\tp{3}$ and each $\lambda_i > 0$. If 
%  \begin{align}
%    \epsilon &\le O(\frac{\lambda_{min}}{k}) \\
%    N &\ge O(\log(k) + \log \log(\frac{ \lambda_{max} }{\epsilon} ), 
%  \end{align}
%  and for $L = O( poly(k) \log(\frac{1/\eta}) )$  attempts, then with
%  probability at least $1 - \eta$, there exists a permutation $\pi$ on
%  $[k]$ such that,
%  \begin{align}
%    \|v_{\pi(j)} - \hat v_j\| &\le 8 \epsilon/\lambda_{\pi(j)} \\
%    \|\lambda_{\pi(j)} - \hat \lambda_j\| &\le 5 \epsilon.
%  \end{align}
%\end{lemma}
%\begin{proof}
%  \cite{AnandkumarGeHsu2012}
%\end{proof}

%\todo{ This only gives us the eigenvectors for an orthogonal
%decomposition. We also need to work out the darned coefficients
%whitening the tensor adds.  Namely, what is $\delta T(W,W,W)$ (for which
%the above bound applies), given $\delta W$ and ultimately $\delta P$
%($W^T P W = I$). These calculations can be found in the notes I had had
%earlier.}
%

